The quantum origins of the cosmological asymmetry

The standard inflationary version of the origin of the cosmic structure as the result of the quantum fluctuations during the inflationary stage is less than fully satisfactory: how exactly does the Universe transit from a homogeneous and isotropic stage to one where the quantum uncertainties become actual inhomogeneous fluctuactions? The point is that the predictions of inflation in this regard cannot be fully justified in any known scheme of quantum physics. A proposal was made in [A. Perez, H. Sahlmann and D. Sudarsky, Classical and Quantum Gravity 23, 2317 (2006)] to solve this problem by invoking a process similar to the collapse of the quantum mechanical wave function of the various modes of the inflaton field. This in turn was inspired by ideas of R. Penrose about the roles that quantum gravity might play in bringing about such breakdown of standard unitary evolution of quantum mechanics. In this work we propose and study a new collapse scheme that follows the correlations indicated in the Wigner functional of the initial state. Furthermore, in his thesis work we will focus on a more detailed study of three collapse schemes (robustness, multiple collapses) and on the traces they might leave on the observational data.

==> spanishbst.tex <==
\def\bbland{y}                   
\def\bbleditors{editores}        
\def\bbleditor{editor}           
\def\bbledby{editado por}
\def\bbledition{\,edici\'on}       
\def\bblvolume{volumen}          
\def\bblof{de}
\def\bblnumber{n\'umero}           
\def\bblin{en}
\def\bblpages{p\'aginas}           
\def\bblpage{p\'agina}             
\def\bblchapter{cap\'itulo}    
\def\bbltechreport{Informe t\'ecnico}
\def\bblmthesis{Tesina o Proyecto}
\def\bblphdthesis{Tesis doctoral}
\def\bblfirst{Primer}
\def\bblsecond{Segundo}
\def\bblthird{Tercero}
\def\bblfourth{Cuarto}
\def\bblfifth{Quinto}            
\def\bblst{ª}      
\def\bblnd{ª}  
\def\bblrd{ª}
\def\bblth{th}
\def\bbljan{Enero}    
\def\bblfeb{Febrero}    
\def\bblmar{Marzo}
\def\bblapr{Abril}    
\def\bblmay{Mayo}       
\def\bbljun{Junio}
\def\bbljul{Julio}    
\def\bblaug{Agosto}     
\def\bblsep{Septiembre}
\def\bbloct{Octubre}  
\def\bblnov{Noviembre}  
\def\bbldec{Diciembre}
\def\bibcommentname{Notas:}
\def\bbletal{y otros}
\def\bbleds{eds.}    
\def\bbled{ed.}      
\def\bbledn{ed.}     
\def\bblvol{vol.}    
\def\bblno{n\'um.}     
\def\bblpp{pp.}      
\def\bblp{p.}        
\def\bblchap{cap.}   
\def\bibtranslatorname{Traducido por }

